Stock Selection as a Problem in Phylogenetics -- Evidence from the ASX

We report the results of fifteen sets of portfolio selection simulations using stocks in the ASX200 index for the period May 2000 to December 2013. We investigated five portfolio selection methods, randomly and from within industrial groups, and three based on neighbor-Net phylogenetic networks. We report that using random, industrial groups, or neighbor-Net phylogenetic networks alone rarely produced statistically significant reduction in risk, though in four out of the five cases in which it did so, the portfolios selected using the phylogenetic networks had the lowest risk. However, we report that when using the neighbor-Net phylogenetic networks in combination with industry group selection that substantial reductions in portfolio return spread were achieved.

==> Methods.tex <==
\section{Methods}\label{sec:methods}

\subsection{Neighbor-Net Splits Graphs}

To be able to use clustering algorithms (neighbor-Net is a
clustering algorithm) 
we
need to convert the numerical values in the correlation matrix to
a measure which can be used as a distance. In the
literature the most common way to do the conversion is
by using the so-called ultra-metric, 
\begin{equation}
d_{ij}=\sqrt{2(1-\rho_{ij})} \label{eqn:sqrt1mc} 
\end{equation}
where $d_{ij}$ is the distance corresponding to the
the estimated correlation, $\rho_{ij}$, between stocks $i$ and $j$,
see \cite{Mantegna1999} or  \cite{Djauhari2012}
for details.

A typical stock market correlation matrix for $n$ stocks
 is of full rank which means 
that after converting to a distance matrix according to
Equation \eqref{eqn:sqrt1mc}, the location of the points,
here stocks, 
it can only be represented fully in an $(n-1)$-dimensional
space. Some basic statistics on the correlations are
presented in Table (\ref{tab:basicstats}).
In visualization, the high dimensional data space is collapsed
to a sufficiently low dimensional space that the
data can be
represented on 2-dimensional surface such as a page or computer
screen for viewing. Information loss is often unavoidable
in the reduction of the dimension of the data space.  One
of the goals of visualization is to minimize the information
loss while making the structures within the data visible to the
human eye.

Using the conversion in Equation \eqref{eqn:sqrt1mc} we formatted
the converted correlation matrix and 
augmented it with the appropriate stock codes for reading into
the neighbor-Net software, SplitsTree, available from
 \verb+http://www.splitstree.org+. Using the SplitsTree software
we generated the neighbor-Nets splits graphs. Because the splits
graphs are intended to be used for visualization we defer the
discussion of the identification of correlation clusters and
their uses to Sections (\ref{sec:clusters}) and (\ref{sec:movements})
below.



\subsection{Simulated Portfolios}

Recently \cite{Lee2011} discussed so-called risk-based asset
allocation (sometimes called risk budgeting). 
In contrast to strategies which require both
expected risk and expected returns for each investment opportunity
as inputs to the portfolio selection process, 
risk-based
allocation considers only expected risk. The four methods 
of portfolio selection we
present below can be considered to be risk-based allocation methods.
This probably reflects private investor behaviour in that often they
have nothing more than broker buy, hold, or sell recommendations
to assess likely returns.

The four portfolio methods were compared using simulations. For each of 1,000 iterations a portfolio was sampled based on the rules governing the 
portfolio type. We recorded at the mean and standard deviation of the returns 
for the 1,000 portfolios. 


As mentioned in the introduction the primary motivation is to investigate four portfolio strategies. These are:
\begin{enumerate}
\item Selecting stocks at random;
\item Selecting stocks based on industry groupings;
\item Selecting stocks based on correlation clusters; and
\item Selecting stocks based on industry groups within correlation clusters.
\end{enumerate}
We describe each of these in turn.

\begin{description}
\item[Random Selection: ]
The stocks were selected at random using a uniform distribution without 
replacement. In other words each stock was given equal chance of 
being selected according but with no stock being selected twice within a 
single portfolio. 

\item[By Industry Groups: ]
There were 11 industry groups represented among the stocks. 
Some of the groups were very small, for example, the telecomminications 
group only had two representatives. Thus it was necessary to merge
some of the smaller groups into larger groups for the
purposes of the simulations. Given that the maximum portfolio
size simulated was eight stocks, we required a maximum of eight groups.


% from other paper, needs updating.

If the portfolio size was five or 
less, the industries were chosen at random using a 
uniform distribution without replacement.
From each of the selected industry groups one stock was selected. 
If the desired portfolio size was more than five then each group had at 
least $s$ stocks selected, where $s$ is the quotient of the portfolio 
size divided by five. Some (the remainder of the portfolio size divided by five) industry groups will have $s+1$ stocks selected and the industry groups this applied to were chosen using a uniform distribution without
replacement. Within each industry group stocks were selected using
a uniform distribution, again without replacement.
%Because there were only a few stocks selected from each industry group, portfolios with a stock selected twice remained in the sample. 
%% if we do want to check for stock double up I can add this to the code

\item[By Correlation Clusters: ]
%As described above, the neighbor-Net diagrams are constructed from a distance matrix and represent the correlation structure. The LASSO algorithm for determining which splits are essential to represent the distances, returns an ordering of the splits, from the first to be included to the last. This ordering excludes any splits which were added in an iteration but later removed. This ordering provides a basis for determining eligible clusters.

%Many of the splits are trivial splits, those separating one taxa (stock) from the rest. Some splits separate small clusters of stocks from the remainder. These small clusters are likely to be too small to contain meaningful correlation clusters. Therefore an eligible correlation cluster is defined as a cluster larger than the cutoff value. In this paper we used 25\% of the total number of stocks as the cutoff (rounded down). 

%Each eligible cluster is defined by a split, or bipartition of the stocks. In this paper only the smaller bipartition was considered. The clusters can overlap and often have many stocks in common. The eligible clusters are ordered, essential for investigating the effect of varying portfolio size.

%Description above is for statistical clusters, we have used by eye

The correlation clusters were determined by examining the neighbor-Net network for the relevant periods (period one, two and three). Each stock was assigned to exactly one cluster and each cluster can be defined by a single split (or bipartition) of the circular ordering of the neighbor-Net of the relevant period. The clusters determined in periods one, two and three were used to generate the portfolios for out-of-sample
testing in periods two, three and four respectively. Because the
goal of portfolio building is to reduce risk each cluster was paired
with another cluster which was considered most distant from it.
This method is discussed in detail below.

As with the industry groups, if there were fewer clusters than the desired portfolio size, cluster pairs were selected at random and a stock selected from within each correlation cluster pair. 
If the desired portfolio size was larger than the number of correlation cluster then we apply the method described above for the industry clusters.

As indicated above each cluster was paired with the one most distant
from it. Because we identified
an even number of clusters in period two, cluster one was paired
with cluster five, two with six and so on. In periods with an
odd number of clusters the pairing may not be so straight-forward.
For example, in period two (see Figure \ref{fig:ChinaP2ClCC})
we identified five clusters and
cluster one was paired with four, both clusters two and three
were paired with five, four was paired with one and five with two.


\item[By Dominant or Non-Dominant Industry Group within Correlation Clusters: ]
The final two methods were selecting stocks from industry groups within 
correlation clusters. Each stock within each  cluster has an associated 
industry group. Therefore each correlation cluster can be subdivided into 
up to nine sub-clusters based on industry. However, it is clear that
in a number of clusters one industry was dominant, sometimes more
than half of the stocks within a cluster were from the same industry
group. This lead us to assign each stock to either the dominant
industry group or the non-dominant industry groups creating two groups
of stocks within each cluster. This created two disjoint sets of 
clusters with no stock in both groups.

From these two sets of simulations were run in the same manner as that
described in ``By Correlation Clusters'' above. These simulations were
not comparable with the three above because the same sizes were different
and, obviously, each deals with a subset of the data. However, care was
taken to ensure that the sample sizes of both subsets was as close to
equal in size as was practical. 

A problem arose, particularly with the non-dominant industry group
stocks in that the number of stocks in the cluster was considered
too small. In these cases we took advantage of the circular ordering
produced by neighbor-Nets and combined the small cluster with a 
neighbouring cluster. 


Unchanged from above, each cluster was paired with the one most distant
from it. Once a cluster was selected for inclusion, so was the paired cluster,
and a selection was made using a uniform distribution and, if necessary, without
replacement.


\end{description}
All simulations were coded and run in R \citep{R}.


==> NNets.tex <==
\section{Neighbor-Net}\label{ssec:nnet}

In this appendix we give a descriptive overview of the Neighbor-Net algorithm 
and the splits graphs (see Figure \ref{fig:NZX_Magnified} for an 
example) it produces. The \ref{app:neighbornet} contains the technical details.

The Neighbor-Net algorithm was a further development of
an algorithm for phylogenetic tree construction
advanced by \cite{Saitou1987}. 
Neighbor-Net was developed to represent the relationships between DNA strands once each pair of genetic sequences was converted to a distance measure. Neighbor-Net takes a matrix of pairwise distances and produces a network,
or splits graph,
based on ``splits''. A split is a partition of the set of nodes (in our case companies on the stock exchange) into two disjoint, non-empty groups.  

Because the input for the Neighbor-Net algorithm  is a matrix
of pairwise distances,
the Neighbor-Net algorithm is
a type of clustering algorithm and 
can be applied to any distance matrix. 
Typically the most important information generated by Neighbor-Net
is the location of the node on the periphery. 
Additionally, some of the bifurcations may represent key differences between
the two groups. These two types of information yield insights into correlations in stock markets.


A splits graph need not be planar and is not necessarily unique,
but \cite{Bryant2004} state ``the splits graphs generated by Neighbor-Net are 
{\em always} planar, an important advantage over other network
methods when it comes to visualization'' (emphasis original).

The Neighbor-Net algorithm is implemented in SplitsTree and is available
from \verb+http://www.splitstree.org+ \citep{Huson2006}.



==> Notes.tex <==
\section*{Notes On Paper -- Not for inclusion in the final version}

\subsection{NN Diagrams}

All the \verb+nex+ files for the NN diagrams are in the subdirectories off
\begin{verbatim}
~/Dropbox/Hannah Master/ASX200 Split into 6 periods
\end{verbatim}
The taxa groups have been put into the data menu.

\subsection{Simulations}

All the code for the simulations are in the directory
\begin{verbatim}
~/Dropbox/Hannah Master/ASX200 Split into 6 periods/Code 13 Jan 2014
\end{verbatim}
The individual simulation files are named ASX200Period2.R to 
ASX200Period6.R for the out-of-sample testing. Currently there is no
in-sample, but that could be changed easily if required once the groups 
are sorted out.

I created a directory
\begin{verbatim}
~/Dropbox/Hannah Master/ASX200 Split into 6 periods/SortingStocks
\end{verbatim}
for working on issues of which stocks have data and so should be included
in the simulations.


